Acceleration of Sparse and Irregular Workloads through Energy-Efficient Stream Extensions

The slowdown of Moore's law and Dennard scaling has motivated computer architects to uphold performance scaling through architectural specialization. So far, most efforts have focused on highly regular workloads, which exhibit good data locality, ample reuse, and a data-independent execution flow. As this specialization hits diminishing returns, attention shifts towards sparse and irregular workloads, which are essential to applications like sparse neural networks, multiphysics simulations, and graph analytics. However, they lack the convenient properties of highly regular compute that modern architectures are optimized for, resulting in very low (<10%) functional unit utilization on traditional CPUs and GPUs. The most promising approaches to their general hardware acceleration leverage memory streams, which decouple data movement from execution. In this thesis, we explore energy-efficient hardware stream extensions that significantly accelerate sparse and irregular workloads in general-purpose systems without specializing to specific application domains or compromising on regular-workload performance. We design a flexible, core-coupled stream extension supporting affine and indirect streams as well as intersection and union of sparse tensors. We integrate it into an energy-efficient RISC-V compute cluster, achieving significant performance and energy efficiency benefits on general sparse linear algebra, and further use it to accelerate stencil computations, spiking neural network inference, and model-predictive control. We evaluate it at scale in a 432-core 2.5D RISC-V system fabricated in 12nm FinFET, achieving leading compute utilization and energy efficiency on sparse and irregular workloads while remaining competitive on regular workloads. Finally, we extend chip-level interconnects with end-to-end irregular streams, improving performance, energy efficiency, and bus utilization.

==> IISthesis_title_back.tex <==
\null

{\scriptsize
In reference to IEEE copyrighted material which is used with permission in this thesis, the IEEE does not endorse any of ETH Zurich's products or services.
Internal or personal use of this material is permitted.
If interested in reprinting/republishing IEEE copyrighted material for advertising or promotional purposes or for creating new collective works for resale or redistribution, please go to \url{http://www.ieee.org/publications_standards/publications/rights/rights_link.html} to learn how to obtain a License from RightsLink.
If applicable, University Microfilms and/or ProQuest Library, or the Archives of Canada may supply single copies of the dissertation.
}

